Selective Feature Adapter for Dense Vision Transformers

Fine-tuning pre-trained transformer models, e.g., Swin Transformer, are successful in numerous downstream for dense prediction vision tasks. However, one major issue is the cost/storage of their huge amount of parameters, which becomes increasingly challenging to handle with the growing amount of vision tasks. In this paper, we propose an effective approach to alleviate the issue, namely selective feature adapter (SFA). It achieves state-of-the-art (SoTA) performance under any given budget of trainable parameters, and demonstrates comparable or better performance than fully fine-tuned models across various dense tasks. Specifically, SFA consists of external adapters and internal adapters which are sequentially operated over a transformer model. For external adapters, we properly select the places and amount of additional multilayer perception (MLP). For internal adapters, we transform a few task-important parameters inside the transformer, which are automatically discovered through a simple yet effective lottery ticket algorithm. Our experiments show that the dual adapter module, a.k.a SFA, is essential to achieve the best trade-off on dense vision tasks, such as segmentation, detection and depth-estimation, outperforming other adapters with a single module.

==> 3-method-peng.tex <==
\subsection{Internal Feature adapter $\mathcal{F}_i$}
\label{subsec:internal}
In this section, we elaborate $\mathcal{F}_i$ which further adapts important parameters inside the transformer $\mathcal{T}$. 

That is motivated by our observation, as also introduced in Sec.~\ref{sec:intro}, that on dense prediction tasks like segmentation, the performance with simple external adaptor is saturated with a gap matching the fully-finetuned model, no matter how large we set the MLP dimension $d$. Therefore, we believe there must be some important feature representation internally that is necessary to be discovered. 

Specifically, $\mathcal{F}_i$ tries to adapt feature in both MH-Att and MLP.  


We derive a parameter calculation method. We surprisingly find some parameters are commonly significants, and these parameters could be used to transfer the knowledge from the pre-trained model to downstream tasks efficiently.
We only update features of these parameters with high importance scores. This design enables us to tune only a subset of parameters
instead of all, inheriting the strong representations of pretrained backbones for downstream tasks. For different downstream datasets, the selected important parameters in each layer are different, and it could explicitly involve dataset-specific information into the model adaptation.

% \begin{comment}
    
% delta mathmatical function
% 1(delta) = True

% 1000 --> T1
% 2000 --> T2
% 3000 --> T3
% 4000 --> T4

% \end{comment}


Given the importance score to select top-K important parameters, it is natural to tune only these parameters for efficient model tuning, named as xxx in this paper. Unlike other parameter-efficient tuning methods, our xxx only contains 


Discussion. We address two critical problems for adapting the large ViT models to downstream tasks, namely, avoiding overfitting and reducing the number of trainable parameters. We find that the state-of-the-art baselines lack the consideration of explicitly using the dataset-specific information. Moreover, different downstream tasks have their own peculiarities, i.e., “Not all parameters are equal”. Thus, we propose the xxx to explicitly incorporate the dataset-specific information in the model tuning, which could achieve better results and simultaneously reduce the parameters. Moreover, calculating the important parameters  could save the computations of searching the best prompt length as in VPT or the best network structure as in NOAH.


%Metric/higher score/Whole-model


We consider the training of a non-convex loss function. We assume for a weight vector w to have access to a stochastic gradient g(w). This corresponds to the standard machine learning setting with g(w) representing a (mini-batch) gradient of one (or several) components of the loss function. Stochastic Gradient Descent (SGD) computes a sequence of iterates by the update rule.
To obtain a sparse model, a general approach is to prune some of the weights of wt, i.e., to set them to zero. Such pruning can be implemented by applying a mask to the weights, resulting in a sparse model. The mask could potentially depend on the weights wt (e.g., smallest magnitude pruning), or depend on t (e.g., the sparsity is incremented over time).




%Only draw our method network
%Motivation
%Discussion

% \begin{comment}
    
\begin{algorithm}[tb]
\caption{Our xxx}
\label{alg:algorithm}
\textbf{Input}: 
Full train data set $\mathcal{D}$; Initialization of $\alpha_0$, $\theta_0$; Number of iterations $T_{search}$ and $T$.\\
\textbf{Output}: Trained student.
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Split $D$ into $D_{train}$ and $D_{val}$.
\STATE Let $t=0$.
\WHILE{$t < T_{search}$}
\STATE Compute $\alpha_t$ with descending the gradient approximation in Eq.~\ref{eq:final} and do normalization.
\STATE Update $\theta_t$ by descending $\nabla_\theta L_{train}(\theta_t; \alpha_t)$ in Eq.~\ref{eq:alphatrain}.
\STATE Push the current $\alpha_t$ to $\mathcal{A}$.
\ENDWHILE
\STATE Interpolate $\mathcal{A}$ with length of $T$.
\STATE Set $D_{train} = D$ or use a new $D_{train}$ in another task.
\STATE Reset $t = 0$.
\WHILE{$t < T$}
\STATE Load the $\alpha_t$ corresponding to the current $t$. \label{algo:line:load}
\STATE Update $\theta$ by descending $\nabla_\theta L_{train}(\theta, \alpha_t)$.
\ENDWHILE
\end{algorithmic}
\end{algorithm}
% \end{comment}






Pruning during training (incremental and dynamic pruning). Dynamic schemes change the mask mt every (few) iterations based on observations during training (i.e. by observing the weights and stochastic gradients). Incremental schemes monotonically increase the sparsity pattern, fully dynamic schemes can also reactivate previously pruned weights. In contrast to previous dynamic schemes that relied on elaborated heuristics to adapt the mask mt, we propose a simpler approach:

Dynamic pruning with feedback. Our scheme evaluates a stochastic gradient at the pruned model and applies it to the (simultaneously maintained) dense model.
Applying the gradient to the full model allows to recover from “errors”, i.e. prematurely masking out important weights: when the accumulated gradient updates from the following steps drastically change a specific weight, it can become activated again (in contrast to incremental pruning approaches that have to stick to sub-optimal decisions). 

\subsection{Training Trainable Weights}

Gradual training

The weight magnitude analysis motivates us not to fix the trainable parameters too early. 
It is also implied that a distance-based metric might not reveal the winning structure of the model at different epochs. To understand the early winning structures, we further investigate the impact of the sparsified structure on the final accuracy. Considering that a highly pruned network is likely to have limited learning capability, we make a conjecture that the accuracy degradation of a
pruned model is due to the loss of capability for learning complex pattern if pruned too early. Recently, some works reveal that the training behavior of a sufficiently over-parameterized model with non-linearity highly depends on the learning rate schedule, where a model tends to memorize the complex patterns when a small learning rate is applied while learning simple patterns with a large learning rate. To validate this claim in the context of pruning, we construct an experiment where a model is pseudo-pruned at every epoch of the baseline training then retrained with large or small learning rate for just one epoch. %For the pseudo-pruned-then-retrained (PPR) model at each baseline epoch, we measure the validation accuracy recovered from the retraining.

The reasoning behind the gradual pruning is that the model can be changed graciously if the pruning is applied gradually. In terms of the early winning ticket analysis, there are two factors playing the critical role: 1) by applying low pruning rate in the beginning, the structure found at that pruning level can preserve the memorization capacity better, 2) once pruning is applied, the remaining weights of the pruned model is updated via SGD, granting a chance for the pruned
model to adopt its weights toward better accuracy. Thanks to these two factors, a structure with better memorization capacity can be found when the increased pruning rate is applied next time.



\begin{comment}
\subsection{Dual Adapter Network}

\subsubsection{Discussion}
\begin{itemize}
    \item Difference with other weight adapters
    \item Difference with model pruning methods
    \item Difference with other feature adapters (VPT, adapterformer)
\end{itemize}

\end{comment}

\textbf{Other alternatives.} 
Pruning before training. A mask m0 (depending on e.g. the initialization w0 or the network architecture of f) is applied and (SGD) is used for training on the resulting subnetwork with the advantage that only pruned weights need to be stored and updated, and that by training with SGD a local minimum of the subnetwork can be reached. In practice however, it remains a challenge to efficiently determine a good mask m0 and a wrongly chosen mask at the beginning strongly impacts the performance.

Pruning after training (one-shot pruning). A dense model is trained, and pruning is applied to the trained model. As the pruned model is very likely not at a local optimum of f, fine-tuning (retraining with the fixed mask) is necessary to improve performance.  

